A Case For Amplify-Forward Relaying in the Block-Fading Multi-Access Channel

This paper demonstrates the significant gains that multi-access users can achieve from sharing a single amplify-forward relay in slow fading environments. The proposed protocol, namely the multi-access relay amplify-forward, allows for a low-complexity relay and achieves the optimal diversity-multiplexing trade-off at high multiplexing gains. Analysis of the protocol reveals that it uniformly dominates the compress-forward strategy and further outperforms the dynamic decode-forward protocol at high multiplexing gains. An interesting feature of the proposed protocol is that, at high multiplexing gains, it resembles a multiple-input single-output system, and at low multiplexing gains, it provides each user with the same diversity-multiplexing trade-off as if there is no contention for the relay from the other users.

==> rv_defs.tex <==
%% Definitions of random variable fonts.


\DeclareMathAlphabet{\mathbsf}{OT1}{cmss}{bx}{n}% bold sans serif
\DeclareMathAlphabet{\mathssf}{OT1}{cmss}{m}{sl}% slanted sans serif
\DeclareMathAlphabet{\mathcsf}{OT1}{cmss}{sbc}{n}% condensed sans serif


% define some useful uppercase Greek letters in regular and bold sf
\DeclareSymbolFont{bsfletters}{OT1}{cmss}{bx}{n}
\DeclareSymbolFont{ssfletters}{OT1}{cmss}{m}{n}
\DeclareMathSymbol{\bsfGamma}{0}{bsfletters}{'000}
\DeclareMathSymbol{\ssfGamma}{0}{ssfletters}{'000}
\DeclareMathSymbol{\bsfDelta}{0}{bsfletters}{'001}
\DeclareMathSymbol{\ssfDelta}{0}{ssfletters}{'001}
\DeclareMathSymbol{\bsfTheta}{0}{bsfletters}{'002}
\DeclareMathSymbol{\ssfTheta}{0}{ssfletters}{'002}
\DeclareMathSymbol{\bsfLambda}{0}{bsfletters}{'003}
\DeclareMathSymbol{\ssfLambda}{0}{ssfletters}{'003}
\DeclareMathSymbol{\bsfXi}{0}{bsfletters}{'004}
\DeclareMathSymbol{\ssfXi}{0}{ssfletters}{'004}
\DeclareMathSymbol{\bsfPi}{0}{bsfletters}{'005}
\DeclareMathSymbol{\ssfPi}{0}{ssfletters}{'005}
\DeclareMathSymbol{\bsfSigma}{0}{bsfletters}{'006}
\DeclareMathSymbol{\ssfSigma}{0}{ssfletters}{'006}
\DeclareMathSymbol{\bsfUpsilon}{0}{bsfletters}{'007}
\DeclareMathSymbol{\ssfUpsilon}{0}{ssfletters}{'007}
\DeclareMathSymbol{\bsfPhi}{0}{bsfletters}{'010}
\DeclareMathSymbol{\ssfPhi}{0}{ssfletters}{'010}
\DeclareMathSymbol{\bsfPsi}{0}{bsfletters}{'011}
\DeclareMathSymbol{\ssfPsi}{0}{ssfletters}{'011}
\DeclareMathSymbol{\bsfOmega}{0}{bsfletters}{'012}
\DeclareMathSymbol{\ssfOmega}{0}{ssfletters}{'012}


%% Random variable/vector declarations.  Please add in alphabetical
%% order.  First section is for capitals.  Second for lower case.
\newcommand{\rvA}{{\mathssf{A}}}    % A
\newcommand{\rvbA}{{\mathbsf{A}}}
\newcommand{\rvB}{{\mathssf{B}}}
\newcommand{\rvbB}{{\mathbsf{B}}}
\newcommand{\rvC}{{\mathssf{C}}}
\newcommand{\rvF}{{\mathssf{F}}}
\newcommand{\rvH}{{\mathssf{H}}}
\newcommand{\rvI}{{\mathssf{I}}}
\newcommand{\rvL}{{\mathssf{L}}}    % L
\newcommand{\rvM}{{\mathssf{M}}}    % M
\newcommand{\rvN}{{\mathssf{N}}}    % N
\newcommand{\rvR}{{\mathssf{R}}}    % R
\newcommand{\rvS}{{\mathssf{S}}}    % S
\newcommand{\rvW}{{\mathssf{W}}}    % W
\newcommand{\rvX}{{\mathssf{X}}}    % X
\newcommand{\rvY}{{\mathssf{Y}}}    % Y
\newcommand{\rvZ}{{\mathssf{Z}}}    % Z

\newcommand{\rva}{{\mathssf{a}}}    % a
\newcommand{\rvba}{{\mathbsf{a}}}
\newcommand{\rvb}{{\mathssf{b}}}    % b
%\newcommand{\rvbh}{\hat{\rvb}}
\newcommand{\rvc}{{\mathssf{c}}}    % c
\newcommand{\rvbc}{{\mathbsf{c}}}
\newcommand{\rvd}{{\mathssf{d}}}    % d
\newcommand{\rvbd}{{\mathbsf{d}}}
\newcommand{\rve}{{\mathssf{e}}}    % e
\newcommand{\rvbe}{{\mathbsf{e}}}
\newcommand{\rvf}{{\mathssf{f}}}    % f
\newcommand{\rvg}{{\mathssf{g}}}
\newcommand{\rvh}{{\mathssf{h}}}    % h
\newcommand{\rvbh}{{\mathbsf{h}}}
\newcommand{\rvk}{{\mathssf{k}}}    % k
\newcommand{\rvl}{{\mathssf{l}}}
\newcommand{\rvm}{{\mathssf{m}}}    % m
\newcommand{\rvmh}{\hat{\rvm}}
\newcommand{\rvbm}{{\mathbsf{m}}}
\newcommand{\rvbmh}{\hat{\rvbm}}
\newcommand{\rvn}{{\mathssf{n}}}    % n
\newcommand{\rvbn}{{\mathbsf{n}}}
\newcommand{\rvq}{{\mathssf{q}}}    % q
\newcommand{\rvr}{{\mathssf{r}}}    % r
\newcommand{\rvs}{{\mathssf{s}}}    % s
\newcommand{\rvsh}{\hat{\rvs}}
\newcommand{\rvbs}{{\mathbsf{s}}}
\newcommand{\rvt}{{\mathssf{t}}}    % t
\newcommand{\rvu}{{\mathssf{u}}}    % u
\newcommand{\svu}{{u}}
\newcommand{\svbu}{{\mathbf{u}}}
\newcommand{\rvbu}{{\mathbsf{u}}}
\newcommand{\rvv}{{\mathssf{v}}}    % v
\newcommand{\svv}{{v}}
\newcommand{\rvbv}{{\mathbsf{v}}}
\newcommand{\svbv}{{\mathbf{v}}}
\newcommand{\rvw}{{\mathssf{w}}}    % w
\newcommand{\svw}{{w}}
\newcommand{\rvbw}{{\mathbsf{w}}}
\newcommand{\svbw}{{\mathbf{w}}}
\newcommand{\rvwh}{\hat{\rvw}}
\newcommand{\rvx}{{\mathssf{x}}}    % x
\newcommand{\rvxh}{\hat{\rvx}}
\newcommand{\rvbx}{{\mathbsf{x}}}
\newcommand{\rvy}{{\mathssf{y}}}    % y
\newcommand{\rvyh}{{\hat{\rvy}}}
\newcommand{\rvby}{{\mathbsf{y}}}
\newcommand{\rvz}{{\mathssf{z}}}    % z
\newcommand{\rvzh}{\hat{\rvz}}
\newcommand{\rvbz}{{\mathbsf{z}}}

% Handle uppercase Greek differently
\newcommand{\rvDelta}{\ssfDelta}
\newcommand{\rvbDelta}{\bsfDelta}
\newcommand{\rvTh}{\ssfTheta}
\newcommand{\rvbTh}{\bsfTheta}
\newcommand{\rvPh}{\ssfPhi}
\newcommand{\rvbPh}{\bsfPhi}

% Caligraphy
%\newcommand{\calp}{{\mathcal{p}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calZ}{{\mathcal{Z}}}

